EUGENE: Explainable Structure-aware Graph Edit Distance Estimation with Generalized Edit Costs

The need to identify graphs with small structural distances from a query arises in domains such as biology, chemistry, recommender systems, and social network analysis. Among several methods for measuring inter-graph distance, Graph Edit Distance (GED) is preferred for its comprehensibility, though its computation is hindered by NP-hardness. Optimization based heuristic methods often face challenges in providing accurate approximations. State-of-the-art GED approximations predominantly utilize neural methods, which, however: (i) lack an explanatory edit path corresponding to the approximated GED; (ii) require the NP-hard generation of ground-truth GEDs for training; and (iii) necessitate separate training on each dataset. In this paper, we propose EUGENE, an efficient, algebraic, and structure-aware optimization based method that estimates GED and also provides edit paths corresponding to the estimated cost. Extensive experimental evaluation demonstrates that EUGENE achieves state-of-the-art GED estimation with superior scalability across diverse datasets and generalized cost settings.

==> sections/03.4.properties.tex <==
\subsection{Properties of \name}

%In this section, we list the important properties of \name. 
\begin{comment}
\begin{theorem}
\label{thm:convergence}
\pk{\textsc{M-Adam} (Alg.~\ref{M-Adam}) converges in finite time.}
\end{theorem}
\vspace{-0.20in} % ugly
\begin{proof}
\pk{Assume \textsc{M-Adam} does not converge for some value of~$\lambda$. Then it must be stuck in the inner $\mathrm{while}$ loop of Algorithm~\ref{M-Adam}. Each iteration of that loop subtracts a fixed positive~$\delta$ from~$\lambda$. In effect, $\lambda$ reaches~0 after finite iterations and remains unchanged thereafter, while the inner $\mathrm{while}$ loop minimizes a convex function, terminating in finite steps. Therefore, \textsc{M-Adam} converges in finite time.\looseness=-1}
%due to the termination of the inner loop.
\end{proof}
\end{comment}
\noindent
\textbf{Interpretable solution:} \pkl{\name yields a permutation matrix (i.e., node mapping) for the estimated GED, thus an edit path from~$\mathcal{G}_{1}$ to~$\mathcal{G}_{2}$; most neural approximators do not do so.}

\noindent
\textbf{Upper bound:} \pkl{As the true GED is the least edit cost over all alignments, the returned GED \emph{upper-bounds} the true GED. Most neural approximators do not yield such a bound.}

\noindent
\textbf{Unsupervised and CPU-bound execution:} \pkl{Unlike neural approximators, \name needs no training data, which is \NPhard to generate. Further, its computation is CPU-bound, offering an environmentally-friendly and lightweight way to approximate GED.}

==> sections/99.references.tex <==
% \section*{Impact Statement}
% This work introduces an efficient algebraic method, \name, to approximate Graph Edit Distance (GED), a critical problem in domains such as biology, chemistry, recommender systems, and social network analysis. Unlike state-of-the-art neural methods, \name eliminates the need for computationally expensive ground truth generation and dataset-specific training, making it accessible and scalable for real-world applications. Furthermore, the method produces explanatory edit paths, enhancing interpretability and transparency, which are vital for applications in sensitive domains such as healthcare and social systems.

% The broader societal impact of this work is positive, as it promotes computational efficiency and interpretable graph analysis without reliance on resource-intensive or opaque neural methods. We do not foresee any ethical concerns arising out of this work.
% \bibliographystyle{ACM-Reference-Format}
\bibliography{references.bib}
% The following commands are available for your use in citing references:
% \begin{quote}
% {\em \textbackslash cite:} Cites the given reference(s) with a full citation. This appears as ``(Author Year)'' for one reference, or ``(Author Year; Author Year)'' for multiple references.\smallskip\\
% {\em \textbackslash shortcite:} Cites the given reference(s) with just the year. This appears as ``(Year)'' for one reference, or ``(Year; Year)'' for multiple references.\smallskip\\
% {\em \textbackslash citeauthor:} Cites the given reference(s) with just the author name(s) and no parentheses.\smallskip\\
% {\em \textbackslash citeyear:} Cites the given reference(s) with just the date(s) and no parentheses.
% \end{quote}
% You may also use any of the \emph{natbib} citation commands.
% \bigskip
% \noindent Thank you for reading these instructions carefully. We look forward to receiving your electronic files!
